Large Area Optical Frequency Detectors for Single-Shot Phase Readout

Attosecond science has demonstrated that electrons can be controlled on the sub-cycle time scale of an optical wave, paving the way toward optical frequency electronics. Using controlled few-cycle optical waveforms, the study of sub-cycle electron emission has enabled the generation of attosecond ultraviolet pulses and the control of attosecond currents inside of solids. However, these experiments rely on high-energy laser systems not suitable for integration with microcircuits. To move towards integrated optical frequency electronics, a system suitable for integration into microcircuits capable of generating detectable signals with low pulse energies is needed. While current from plasmonic nanoantenna emitters can be driven at optical frequencies, low charge yields have been a significant limitation. In this work we demonstrate that large-scale electrically-connected plasmonic nanoantenna networks, when driven in concert, enable a much higher charge yield sufficient for shot-to-shot carrier-envelope phase detection, which is a hallmark of the underlying sub-cycle processes. We use a tailored sub-2-cycle mid-infrared waveform of only tens of nanojoules of energy to drive in excess of 2000 carrier-envelope-phase-sensitive electrons from interconnected plasmonic nanoantenna arrays that we detect on a single-shot basis using conventional electronics. Our work shows that electronically integrated plasmonic nanoantennas are a viable approach to integrated optical frequency electronics. By engineering the nanoantennas to the particular use case, such as carrier-envelope phase detection, and optimizing the density and total amount, the output signals are fully controlled. This approach to optical frequency electronics will further enable many interesting applications, such as petahertz-bandwidth electric field sampling or the realization of logic gates operating at optical frequencies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
